Hierarchical Agglomerative Graph Clustering in Poly-Logarithmic Depth

Obtaining scalable algorithms for hierarchical agglomerative clustering (HAC) is of significant interest due to the massive size of real-world datasets. At the same time, efficiently parallelizing HAC is difficult due to the seemingly sequential nature of the algorithm. In this paper, we address this issue and present ParHAC, the first efficient parallel HAC algorithm with sublinear depth for the widely-used average-linkage function. In particular, we provide a $(1+\epsilon)$-approximation algorithm for this problem on $m$ edge graphs using $\tilde{O}(m)$ work and poly-logarithmic depth. Moreover, we show that obtaining similar bounds for exact average-linkage HAC is not possible under standard complexity-theoretic assumptions. We complement our theoretical results with a comprehensive study of the ParHAC algorithm in terms of its scalability, performance, and quality, and compare with several state-of-the-art sequential and parallel baselines. On a broad set of large publicly-available real-world datasets, we find that ParHAC obtains a 50.1x speedup on average over the best sequential baseline, while achieving quality similar to the exact HAC algorithm. We also show that ParHAC can cluster one of the largest publicly available graph datasets with 124 billion edges in a little over three hours using a commodity multicore machine.

==> geom_bucketing.tex <==
Our starting point is the observation that we can merge \emph{any} pair of vertices
whose similarity is within a $(1+\epsilon)$ factor of the current highest-similarity edge.
This idea motivates \defn{geometric layering}, a technique where we group the edges
into layers based on their weights and process edges in the same layer in parallel (e.g., see ~\cite{Berger1994, BPT11}).
In more detail, let $\mathcal{W}_{\max}$ and $\mathcal{W}_{\min}$ be 
the maximum-weight and minimum-weight in the graph, respectively.
The $i$-th layer contains all edges with
weight between $((1+\epsilon)^{-(i+1)}\cdot \wmax, (1+\epsilon)^{-i} \cdot \wmax]$.
A geometric layering algorithm considers the layers one-by-one, starting
with the heaviest layer and processing all vertices with edges in current layer.
The key challenge is to design an algorithm to process all of the elements
within each layer in few rounds, while ensuring that the algorithm does 
not violate the approximation requirements.


==> seqhac.tex <==
\section{Sequential HAC}\label{sec:seqalg}
In this section we review the
existing exact and $(1+\epsilon)$-approximate sequential HAC algorithms
which are two baselines that we compare against, and also the
starting point for our new theoretical results.

\myparagraph{Exact Average-Linkage}
A challenge in implementing the average-linkage HAC algorithm is to 
efficiently maintain edge weights in the graph as vertices (clusters) are \emph{merged}.
Since the average-linkage formula includes the cluster sizes of both
endpoints of a $(u,v)$ edge when computing the weight of the edge, an algorithm which
eagerly maintains the correct weights of all edges in the graph must update \emph{all} of the
edge weights incident to a newly merged cluster.
Unfortunately one can easily show that even for sparse graphs with $O(n)$ edges, for some graphs this
eager approach requires $\Omega(n^2)$ time.

It was recently shown~\cite{dhulipala2021hierarchical} that exact average-linkage HAC 
algorithm can be implemented in $\tilde{O}(n\sqrt{m})$ time, using the classic 
nearest-neighbor chain technique in conjunction with a low-outdegree orientation data structure. 


\myparagraph{Approximate Average-Linkage (\seqhac{})}
Our parallel algorithm is inspired by the sequential approximate average-linkage HAC algorithm~\cite{dhulipala2021hierarchical}, which runs in near-linear time.
The sequential algorithm uses a lazy strategy to avoid updating
the weights of all edges incident to each merged vertex.
Instead of exactly maintaining the weight of each edge, the algorithm uses
the observation that
the weights of edges incident to a vertex do not need to be updated every single time the cluster represented by this vertex grows.
Namely, if we allow an $(1+\epsilon)^2$-approximate algorithm, the weights of edges incident to a vertex do not need to be updated until the cluster-size of this vertex grows by a multiplicative $(1+\epsilon)$ factor. (The approximation ratio of the algorithm is squared, since the clusters represented by \emph{both} endpoints of an edge may grow by a $(1+\epsilon)$ factor before its weight is updated.)
Since this can happen at most $O(\log_{1+\epsilon} n)$ times, for a constant  $\epsilon$, the overall number of edge weight updates is $\tilde{O}(m)$.

The approximate algorithm adapts the folklore \emph{heap-based} approach
for computing HAC to the approximate setting.
Specifically, the algorithm maintains a heap keyed by the vertices, where the value assigned to a vertex is its current highest-weight incident edge (whose weight is correct up to a $(1+\epsilon)^2$ factor). In each iteration, the highest-weight edge is chosen from the heap and its endpoints are merged.
By setting parameters appropriately one can ensure that the resulting algorithm is  $(1+\epsilon)$-approximate.

